An Empirical Study of Multi-Generation Sampling for Jailbreak Detection in Large Language Models

Detecting jailbreak behaviour in large language models remains challenging, particularly when strongly aligned models produce harmful outputs only rarely. In this work, we present an empirical study of output based jailbreak detection under realistic conditions using the JailbreakBench Behaviors dataset and multiple generator models with varying alignment strengths. We evaluate both a lexical TF-IDF detector and a generation inconsistency based detector across different sampling budgets. Our results show that single output evaluation systematically underestimates jailbreak vulnerability, as increasing the number of sampled generations reveals additional harmful behaviour. The most significant improvements occur when moving from a single generation to moderate sampling, while larger sampling budgets yield diminishing returns. Cross generator experiments demonstrate that detection signals partially generalise across models, with stronger transfer observed within related model families. A category level analysis further reveals that lexical detectors capture a mixture of behavioural signals and topic specific cues, rather than purely harmful behaviour. Overall, our findings suggest that moderate multi sample auditing provides a more reliable and practical approach for estimating model vulnerability and improving jailbreak detection in large language models. Code will be released.

==> sections/related_work.tex <==
\subsection{LLM Safety and Alignment}

Large language models (LLMs) are typically aligned using techniques such as instruction tuning and reinforcement learning from human feedback (RLHF) to reduce harmful or undesirable outputs \citep{Ouyang2022InstructGPT,Bai2022HH}. These approached aim to guide models toward producing helpful and harmless responses by incorporating human preferences into the training process. Despite these efforts, prior work has shown that aligned models remain vulnerable to adversarial manipulation, where carefully crafted prompts can induce the model to generate restricted or harmful content \citep{OpenAI2023GPT4}. This indicates that alignment improves average-case behaviour but does not fully guarantee robustness under adversarial conditions.

\subsection{Jailbreak Attacks}

Jailbreak attacks aim to bypass alignment mechanisms by constructing adversarial prompts that induce models to produce harmful or restricted content. Prior studies demonstrate that such attacks can achieve high success rates even on strongly aligned models, highlighting fundamental limitations in current safety mechanisms \citep{Shen2024DoAnythingNow, Zou2023UniversalJailbreak}. 

A key characteristic of jailbreak attacks is their transferability across models. \citet{Zou2023UniversalJailbreak} show that adversarial prompts can generalise across architectures, suggesting that they exploit shared vulnerabilities rather than model-specific weaknesses. Furthermore, modern jailbreak strategies often rely on prompt rewriting, role-playing, and multi-step reasoning to obscure malicious intent \citep{Yi2024JailbreakSurvey}. Indirect prompt injection attacks further complicate detection by embedding hidden instructions within seemingly benign external content \citep{Greshake2023IndirectPromptInjection}. As a result, harmful intent is increasingly concealed, making detection based solely on surface-level features more challenging.

\subsection{Jailbreak Detection Methods}

Existing jailbreak detection approaches can be broadly categorised based on the information they utilise: prompt-based detection, internal-signal-based detection, and output-based detection \citep{Hu2024GradientCuff, Xie2024GradSafe}.

Prompt-based methods analyse input prompts to identify suspicious patterns or structures associated with jailbreak attempts. While computationally efficient, these approaches are vulnerable to paraphrasing and prompt rewriting, which can preserve malicious intent while altering surface form \citep{Zou2023UniversalJailbreak}. 

Internal-signal-based methods leverage model internals such as hidden states or gradients to support detection. Although these methods can provide richer signals, their applicability is often limited in practice due to restricted access to proprietary model internals \citep{Xie2024GradSafe}. 

Output-based methods focus on analysing generated responses to determine whether harmful behaviour is present. These approaches are widely used in real-world systems, where outputs are often the only observable signal \citep{Chen2025AlmostFree}. However, they typically rely on observable textual features or predefined policies, which may limit their ability to generalise to novel or implicitly expressed harmful behaviours.

\subsection{Output-Level Detection and Its Limitations}

Output-based detection has been explored through both heuristic and statistical approaches. Early work primarily relied on human evaluation and rule-based safety checks as part of alignment pipelines \citep{Bai2022HH, OpenAI2023GPT4}. More recent methods model statistical properties of generated text, including likelihood-based signals and stylistic features \citep{Mitchell2023DetectGPT, Gehrmann2019GLTR, Zellers2019Grover}. 

Lexical-based approaches capture surface-level patterns efficiently but may fail to detect implicitly expressed harmful intent. In contrast, semantic-based methods attempt to capture deeper behavioural signals, such as uncertainty or inconsistency across multiple generations \citep{Kadavath2022Calibration, Sleem2025NegBLEURTForest}. 

Despite these advances, most existing work implicitly assumes a single-output evaluation setting, where only one response per prompt is analysed. This assumption limits the ability of detection systems to capture the full range of model behaviour under adversarial conditions.

\subsection{Stochasticity and Multi-Generation Sampling}

A fundamental property of large language models is their stochastic generation process. Prior work demonstrates that different decoding runs can produce substantially different outputs under identical prompts \citep{Holtzman2020Degeneration}. This variability is further exploited in techniques such as self-consistency, where aggregating multiple generated outputs improves reasoning performance \citep{Wang2023SelfConsistency}. 

These findings suggest that a single output may not be sufficient to represent the full behavioural distribution of a model. In adversarial settings, harmful behaviour may appear only in a subset of generated responses, remaining undetected under single-sample evaluation. Recent work further indicates that semantic inconsistencies across multiple outputs can serve as a useful signal for identifying adversarial behaviour \citep{Sleem2025NegBLEURTForest}. 

Taken together, these observations highlight the importance of considering generation variability when evaluating model safety and jailbreak detection.

\subsection{Research Gap and Position}

Existing work on jailbreak detection has made significant progress in modelling output-level signals. However, most studies evaluate detection performance under a single-output setting, without systematically accounting for generation variability. This limitation may lead to an underestimation of model vulnerability and an incomplete understanding of detection effectiveness. 

In this work, we address this gap by reframing jailbreak detection as a multi-sample auditing problem. Specifically, we investigate how aggregating multiple generations per prompt affects both the observed jailbreak success rate and detection performance. Our study provides a systematic analysis of sampling strategies, cross-model generalisation, and category-level behaviour, offering a more comprehensive evaluation of output-level jailbreak detection.



